Log-Concave Polynomials IV: Approximate Exchange, Tight Mixing Times, and Near-Optimal Sampling of Forests

We prove tight mixing time bounds for natural random walks on bases of matroids, determinantal distributions, and more generally distributions associated with log-concave polynomials. For a matroid of rank $k$ on a ground set of $n$ elements, or more generally distributions associated with log-concave polynomials of homogeneous degree $k$ on $n$ variables, we show that the down-up random walk, started from an arbitrary point in the support, mixes in time $O(k\log k)$. Our bound has no dependence on $n$ or the starting point, unlike the previous analyses [ALOV19,CGM19], and is tight up to constant factors. The main new ingredient is a property we call approximate exchange, a generalization of well-studied exchange properties for matroids and valuated matroids, which may be of independent interest. In particular, given function $\mu: {[n] \choose k} \to \mathbb{R}_{\geq 0},$ our approximate exchange property implies that a simple local search algorithm gives a $k^{O(k)}$-approximation of $\max_{S} \mu(S)$ when $\mu$ is generated by a log-concave polynomial, and that greedy gives the same approximation ratio when $\mu$ is strongly Rayleigh. As an application, we show how to leverage down-up random walks to approximately sample random forests or random spanning trees in a graph with $n$ edges in time $O(n\log^2 n).$ The best known result for sampling random forest was a FPAUS with high polynomial runtime recently found by \cite{ALOV19, CGM19}. For spanning tree, we improve on the almost-linear time algorithm by [Sch18]. Our analysis works on weighted graphs too, and is the first to achieve nearly-linear running time for these problems.

==> preamble.tex <==
\makeatletter


% -- Options

\RequirePackage{options}

\options{
	/opts/.new family,
	/opts/colors/.new toggle=true,
	/opts/fonts/.new toggle=true,
	/opts/math/.new toggle=true,
	/opts/theorems/.new toggle=true,
	/opts/macros/.new toggle=true,
	/opts/graphics/.new toggle=true,
	/opts/tools/.new toggle=true,
	/opts/typesetting/.new toggle=true,
	/opts/biblio/.new toggle=true
}
\options{/opts}

\providetoggle{presentation}
\@ifclassloaded{beamer}{\toggletrue{presentation}}{\togglefalse{presentation}}

% -- Packages

\iftoggle{/opts/math}{
	\RequirePackage{amsmath}
	\RequirePackage{amssymb}
	\RequirePackage{bm}
	\RequirePackage{dsfont}
	\RequirePackage{mathtools}
}{}

\iftoggle{/opts/theorems}{
	\RequirePackage{amsthm}
}{}

\iftoggle{/opts/graphics}{
	\RequirePackage{tikz}
	\RequirePackage{tikz-3dplot}
	\RequirePackage{tcolorbox}
	\RequirePackage{pgfplots}
	\RequirePackage{tcolorbox}
	\pgfplotsset{compat=newest}
}{}

\iftoggle{/opts/tools}{
	\RequirePackage[ruled]{algorithm2e}
	\RequirePackage{datatool}
	\RequirePackage[super]{nth}
	\RequirePackage{scalerel}
	\iftoggle{presentation}{}{
		\RequirePackage[shortlabels]{enumitem}
	}
}{}

\iftoggle{/opts/fonts}{
	\iftoggle{presentation}{}{
		\RequirePackage[sc]{mathpazo}
	}
}{}

\iftoggle{/opts/biblio}{
	\iftoggle{presentation}{}{
		\RequirePackage[backend=biber, style=alphabetic, maxbibnames=99, maxcitenames=99, url=false]{biblatex}
	}
}

\iftoggle{/opts/colors}{
	\newcommand{\declarecolor}[2]{\@ifundefined{\string\color@#1}{\definecolor{#1}{RGB}{#2}\expandafter\newcommand\csname #1\endcsname[1]{\textcolor{#1}{##1}}}{}}
	\declarecolor{Black}{0, 0, 0}
	\declarecolor{White}{255, 255, 255}
	\declarecolor{Gray}{127, 127, 127}
	\declarecolor{LightGray}{216, 216, 216}
	\declarecolor{Orange}{237, 125, 49}
	\declarecolor{LightOrange}{251,229, 214}
	\declarecolor{Yellow}{255, 192, 0}
	\declarecolor{LightYellow}{255, 242, 200}
	\declarecolor{Blue}{91, 155, 213}
	\declarecolor{LightBlue}{222, 235, 247}
	\declarecolor{Green}{112, 173, 71}
	\declarecolor{LightGreen}{226, 240, 217}
	\declarecolor{Navy}{68, 114, 196}
	\declarecolor{LightNavy}{218, 227, 243}
	
	\newcommand{\declareperson}[1]{%
		\expandafter\newcommand\csname#1\endcsname[1]{\textcolor{Orange}{#1: ##1}}%
	}
}{}

\iftoggle{/opts/graphics}{
	\RequirePackage{tikzsymbols}
	
	\usetikzlibrary{decorations}
	\usetikzlibrary{decorations.pathreplacing}
	\usetikzlibrary{decorations.markings}
	\usetikzlibrary{fit}
	\usetikzlibrary{intersections}
	\usetikzlibrary{matrix}
	\usetikzlibrary{overlay-beamer-styles}
	\usetikzlibrary{patterns}
	\usetikzlibrary{shapes}
	\usetikzlibrary{tikzmark}
	\usetikzlibrary{hobby}
	
	\usepgflibrary{arrows.meta}
	
	\tcbuselibrary{skins}
	\tcbuselibrary{raster}
	
	\usepgfplotslibrary{patchplots}
		
	\pgfdeclarelayer{background}
	\pgfdeclarelayer{foreground}
	\pgfsetlayers{background,main,foreground}
	\tikzstyle{na}=[baseline=-0.5ex]
	\tikzset{onslide/.code args={<#1>#2}{%
	  \only<#1>{\pgfkeysalso{#2}}
	}}
	\tikzset{temporal/.code args={<#1>#2#3#4}{%
	  \temporal<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}}{\pgfkeysalso{#4}}
	}}
		
	\pgfplotsset{colormap={WhiteOrange}{
		color=(White)
		color=(Orange)
	}}
	\pgfplotsset{colormap={NavyOrange}{
		color=(LightNavy)
		color=(Orange)
	}}
	\pgfplotsset{colormap={WhiteNavy}{
		color=(White)
		color=(Navy)
	}}
	\pgfplotsset{colormap={WhiteBlack}{
		color=(White)
		color=(Black)
	}}
		
	\newcommand*{\Pic}[2][]{\begin{tikzpicture}\pic[#1]{#2};\end{tikzpicture}}
	\newcommand*{\sPic}[2]{\scalebox{#1}{\Pic{#2}}}
	\newcommand*{\cPic}[2][]{\begin{center}\Pic[#1]{#2}\end{center}}
	
	\newcommand{\rounded}[2][0.7ex]{%
		\begin{tikzpicture}
			\node[inner sep=0ex, draw=White, line width=0ex, opacity=0.] (a) {#2};
			\clip[rounded corners=#1] (a.south west) rectangle (a.north east);
			\node[inner sep=0ex] (a) {#2};
		\end{tikzpicture}%
	}
	
	\newcommand*{\tnode}[2]{\tikzmarknode{#1}{#2}}
}{}

\iftoggle{/opts/typesetting}{
	\iftoggle{presentation}{
	}{
		\RequirePackage{microtype}
		\RequirePackage[noblocks]{authblk}
		\RequirePackage{parskip}
		\RequirePackage{fullpage}
	}
	\RequirePackage{hyperref}
	\RequirePackage[capitalize, nameinlink]{cleveref}
	
	\iftoggle{/opts/colors}{
		\hypersetup{
			colorlinks=true,
			pdfpagemode=UseNone,
			citecolor=Green,
			linkcolor=Navy,
			urlcolor=Black
		}
	}{}
}{}

\iftoggle{/opts/theorems}{
	\iftoggle{presentation}{}{
		\theoremstyle{plain}
		\newtheorem{theorem}{Theorem}
		\newtheorem{lemma}[theorem]{Lemma}
		\newtheorem{corollary}[theorem]{Corollary}
		\newtheorem{proposition}[theorem]{Proposition}
		\newtheorem{fact}[theorem]{Fact}
		\newtheorem{conjecture}[theorem]{Conjecture}
		\newtheorem*{conjecture*}{Conjecture}
		
		\theoremstyle{definition}
		\newtheorem{definition}[theorem]{Definition}
		
		\theoremstyle{remark}
		\newtheorem{remark}[theorem]{Remark}
		\newtheorem{example}[theorem]{Example}
	}
}{}

\iftoggle{/opts/macros}{
	\providecommand{\given}{}
	\newcommand\GivenSymbol[1][]{%
		\nonscript\:#1\vert%
		\allowbreak%
		\nonscript\:%
		\mathopen{}%
	}
	\providecommand{\mid}{}
	\newcommand\MidSymbol[1][]{%
		\nonscript\:#1\|%
		\allowbreak%
		\nonscript\:%
		\mathopen{}%
	}
	\newcommand{\declaredelims}[3]{%
		\expandafter\DeclarePairedDelimiterX\csname#1\endcsname[1]{#2}{#3}{\renewcommand\given{\GivenSymbol[\delimsize]}\renewcommand\mid{\MidSymbol[\delimsize]}##1}%
	}
	
	\declaredelims{set}\{\}
	\declaredelims{card}\lvert\rvert
	\declaredelims{abs}\lvert\rvert
	\declaredelims{norm}\lVert\rVert
	\declaredelims{dotp}\langle\rangle
	\declaredelims{tuple}\lparen\rparen
	\declaredelims{parens}\lparen\rparen
	\declaredelims{bracks}\lbrack\rbrack
	
	\newcommand{\declarenameddelims}[4]{%
		\expandafter\DeclarePairedDelimiterXPP\csname#1\endcsname[1]{#2}{#3}{#4}{}{\renewcommand\given{\GivenSymbol[\delimsize]}\renewcommand\mid{\MidSymbol[\delimsize]}##1}%
		\expandafter\DeclarePairedDelimiterXPP\csname#1X\endcsname[2]{#2_{##1}}{#3}{#4}{}{\renewcommand\given{\GivenSymbol[\delimsize]}\renewcommand\mid{\MidSymbol[\delimsize]}##2}%
	}
	
	
	\let\Pr\relax
	\declarenameddelims{Pr}{\mathbb{P}}\lbrack\rbrack
	\declarenameddelims{Ex}{\mathbb{E}}\lbrack\rbrack
	
	\newcommand*{\eval}[1]{\left.#1\right\rvert}
	
	\iftoggle{presentation}{%
		\newcommand*{\mathdouble}[1]{\mathds{#1}}%
	}{%
		\newcommand*{\mathdouble}[1]{\mathbb{#1}}%
	}
	
	\let\Q\relax
	\newcommand*{\Q}{{\mathdouble{Q}}}
	\let\N\relax
	\newcommand*{\N}{{\mathdouble{N}}}
	\let\Z\relax
	\newcommand*{\Z}{{\mathdouble{Z}}}
	\let\R\relax
	\newcommand*{\R}{{\mathdouble{R}}}
	\let\C\relax
	\newcommand*{\C}{{\mathdouble{C}}}
	\let\1\relax
	\newcommand*{\1}{{\mathds{1}}}
	
	\let\poly\relax
	\DeclareMathOperator{\poly}{poly}
	\DeclareMathOperator{\supp}{supp}
	\DeclareMathOperator{\conv}{conv}
	\DeclareMathOperator{\rank}{rank}
	\let\Im\relax
	\DeclareMathOperator{\Im}{Im}
	\let\Re\relax
	\DeclareMathOperator{\Re}{Re}
}{}
\makeatother


==> stree.tex <==
\section{Sampling Spanning Trees}
\label{sec:strees}

\begin{figure}
\begin{center}
\begin{tikzpicture}
	\pic at (-4, 0) {sptrees={ A/B, B/C, A/D, A/E, E/F, F/G}};
	\begin{scope}[shift={(-4.45, -0.55)}, rotate=50]
		\draw[line width=1, dashed] (0, 0) ellipse (1.2 and 0.3);	
	\end{scope}
	
	\draw[->, line width=1] (-2.5, 0) to node[above, yshift=0.3em] {delete} (-1.5, 0);
	\pic at (0, 0) {sptrees={A/B, B/C, A/D, E/F, F/G}};

	\draw[->, line width=1] (1.5, 0) to node[above, yshift=0.3em] {add} (2.5, 0);
	\pic at (4, 0) {sptrees={A/B, B/C, A/D, E/F, F/G, A/G}};
	\begin{scope}[shift={(4.55, -0.1)}, rotate=-8]
		\draw[line width=1, dashed] (0, 0) ellipse (1 and 0.25);	
	\end{scope}
	\draw[->, line width=1] (4, -1.5) to[bend left=20] node[above] {repeat} (-4, -1.5);
\end{tikzpicture}
\end{center}
\caption{The down-up random walk on spanning trees. An edge of the spanning tree is uniformly at random selected and removed, and then an edge from those connecting the resulting two components is selected uniformly at random and added.}
\label{fig:down-up}
\end{figure}

\begin{figure}
\begin{center}\begin{tikzpicture}
\pic at (-4, 0) {sptrees={A/B, B/C, A/D, A/E, E/F, F/G}};
\begin{scope}[shift={(3.55, -0.55)}, rotate=50]
	\draw[line width=1, dashed] (0, 0) ellipse (1.2 and 0.3);	
\end{scope}
\draw[->, line width=1] (1.5, 0) to node[above, yshift=0.3em] {delete} (2.5, 0);
\pic at (0, 0) {sptrees={A/B, B/C, A/D, E/F, F/G, A/E, A/G}};
\draw[->, line width=1] (-2.5, 0) to node[above, yshift=0.3em] {add} (-1.5, 0);
\pic at (4, 0) {sptrees={A/B, B/C, A/D, E/F, F/G, A/G}};
\begin{scope}[shift={(-3.45, -0.1)}, rotate=-8]
	\draw[line width=1, dashed] (0, 0) ellipse (1 and 0.25);	
\end{scope}
\draw[->, line width=1] (4, -1.5) to[bend left=20] node[above] {repeat} (-4, -1.5);
\end{tikzpicture}\end{center}	
\caption{The down-up random walk on complements of spanning trees. An edge outside of the spanning tree is uniformly at random selected and added, and then an edge from the resulting cycle is uniformly at random picked and removed.}
\label{fig:up-down}
\end{figure}


In this section we prove \cref{thm:spanning-trees}.\footnote{We remark that reliance on \cref{thm:main} in this section is not mandatory and the results of this section would have been possible even without \cref{thm:main}.}

For simplicity of exposition, we first explain the algorithm for sampling uniformly random spanning trees from unweighted graphs $G=(V, E)$, and then explain simple modifications that result in weighted distributions.

Given that the uniform distribution over spanning trees has a log-concave generating polynomial, one could be tempted to run the down-up walk on the set of spanning trees. This is depicted in \cref{fig:down-up}. The random walk is guaranteed to come within an $\epsilon$ distance of the target distribution in $O(\card{V}\log(\card{V}/\epsilon))$ steps by \cref{thm:main}. However the main problem is implementing each step. The first half of the down-up walk is easy; we just need to remove a uniformly random edge from the current spanning tree. However in the second step where we add an edge, we have to potentially look at close to all edges in the graph to see which ones can reconnect the two connected components, and form a spanning tree again. So the overall time complexity would be $O(\card{E}\cdot \card{V}\log(\card{V}/\epsilon))$, which is quadratic in the size of the graph.

Fortunately, the complements of spanning trees also form a matroid, known as the cographic or bond matroid; see \cref{prop:dual,prop:graphic}. Moreover, choosing the complement of a spanning tree uniformly at random is the same as choosing a spanning tree uniformly at random. Note that the cographic matroid is of rank $k=\card{E}-\card{V}+1\leq \card{E}$ and is over a ground set of $\card{E}$ elements. By \cref{thm:main}, the down-up random walk on it, depicted in \cref{fig:up-down}, mixes to within an $\epsilon$ distance of the uniform distribution in time $O(\card{E}\log(\card{E}/\epsilon))$. However here, each step of the down-up random walk can be implemented much more efficiently. In the first half step, we need to select an edge uniformly at random from those not in the spanning tree, and add it to the spanning tree. This can be simply done by maintaining an array of edges not currently in the spanning tree. The more complicated step is detecting the cycle formed by new edge and the tree, and picking a uniformly random edge from it. Fortunately this step can be done in amortized $O(\log \card{E})$ time using dynamic tree data structures such as link-cut trees \cite{ST83}.

Fortunately this random walk has already been studied by \textcite{RTF18}, and details of the link-cut tree operation can be found there. \Textcite{RTF18} simply did not have a tight mixing time bound for the random walk, which we provided here. Since each step takes amortized time $O(\log \card{E})$ and the overal mixing time is $O(\card{E}\log(\card{E}/\epsilon))$, the whole algorithm takes time $O(n\log(n)\log(n/\epsilon))$ where $n$ is the number of edges in the graph.

\paragraph{Weighted Graphs.} In the case of weighted graphs where there is a weight of $w_e$ over every edge $e$, the weighted spanning tree distribution is defined to be
\[ \Pr{T}\propto \prod_{e\in T} w_e. \]
In order to sample from this distribution, it is enough to sample the complement of a spanning tree $E-T$ with inverted edge weights, that is sampling $E-T$ in such a way that
\[ \Pr{E-T}\propto \prod_{e\in E-T}\frac{1}{w_e}. \]
So the down-up random walk for the complement of the spanning tree is modified as follows:
\begin{itemize}
	\item To the current spanning tree $T$, add edge $e\notin T$ selected uniformly at random.
	\item From the edges on the cycle created, select an edge $f$ with probability $\propto 1/w_f$ and remove it.
\end{itemize}
We simply need to modify the sampling procedure to handle the second step above. Fortunately link-cut trees can already do this in the same amortized $O(\log \card{E})$ time \cite{RTF18}.
